Pushing Alias Resolution to the Limit

In this paper, we show that utilizing multiple protocols offers a unique opportunity to improve IP alias resolution and dual-stack inference substantially. Our key observation is that prevalent protocols, e.g., SSH and BGP, reply to unsolicited requests with a set of values that can be combined to form a unique device identifier. More importantly, this is possible by just completing the TCP hand-shake. Our empirical study shows that utilizing readily available scans and our active measurements can double the discovered IPv4 alias sets and more than 30x the dual-stack sets compared to the state-of-the-art techniques. We provide insights into our method's accuracy and performance compared to popular techniques.

==> Makefile <==

# You want latexmk to *always* run, because make does not have all the info.
# Also, include non-file targets in .PHONY so they are run regardless of any
# file of the given name existing.
.PHONY: paper.pdf all clean

# The first rule in a Makefile is the one executed by default ("make"). It
# should always be the "all" rule, so that "make" and "make all" are identical.
all: paper.pdf

# CUSTOM BUILD RULES

# In case you didn't know, '$@' is a variable holding the name of the target,
# and '$<' is a variable holding the (first) dependency of a rule.
# "raw2tex" and "dat2tex" are just placeholders for whatever custom steps
# you might have.

#%.tex: %.raw
#        ./raw2tex $< > $@
#
#%.tex: %.dat
#        ./dat2tex $< > $@

# MAIN LATEXMK RULE

# -pdf tells latexmk to generate PDF directly (instead of DVI).
# -pdflatex="" tells latexmk to call a specific backend with specific options.
# -use-make tells latexmk to call make for generating missing files.

# -interaction=nonstopmode keeps the pdflatex backend from stopping at a
# missing file reference and interactively asking you for an alternative.

paper.pdf:
	latexmk -pdf -pdflatex="pdflatex -f -interaction=nonstopmode" -use-make paper.tex

clean:
	latexmk -CA
	rm -vf *.bbl *.blg *.bcf *.run.xml

source:
	# Needed to create bbl file
	latexmk -pdf -pdflatex="pdflatex -f -interaction=nonstopmode" -use-make paper.tex
	rm -rf source-to-submit
	mkdir -p source-to-submit
	latexpand --verbose --empty-comments paper.tex > source-to-submit/paper.tex
	cp acmart.cls source-to-submit/
	cp ACM-Reference-Format.bst source-to-submit/
	cp paper.bib source-to-submit/
	cp paper.bbl source-to-submit/
	mkdir -p source-to-submit/figures
	cp figures/* source-to-submit/figures/
#	cp $$(egrep '.pdf$$|.png$$' paper.fls | grep -v paper.pdf | cut -d' ' -f2 | sort -u | egrep '^\.') source-to-submit/figures/
	sed -i -E 's+(.*\\includegraphics.*\{).*/(.*)+\1figures/\2+' source-to-submit/paper.tex
	cp Makefile.minimal source-to-submit/Makefile

arxiv: source
	# Apply arxiv note patch
	patch --no-backup-if-mismatch -p1 source-to-submit/paper.tex < arxiv-note.patch

